Flow-edge Guided Video Completion

We present a new flow-based video completion algorithm. Previous flow completion methods are often unable to retain the sharpness of motion boundaries. Our method first extracts and completes motion edges, and then uses them to guide piecewise-smooth flow completion with sharp edges. Existing methods propagate colors among local flow connections between adjacent frames. However, not all missing regions in a video can be reached in this way because the motion boundaries form impenetrable barriers. Our method alleviates this problem by introducing non-local flow connections to temporally distant frames, enabling propagating video content over motion boundaries. We validate our approach on the DAVIS dataset. Both visual and quantitative results show that our method compares favorably against the state-of-the-art algorithms.

==> 5_conclusion.tex <==
\section{Conclusions}
\label{sec:conclusions}

We have presented a new flow-based video completion algorithm capable of synthesizing temporally coherent and visual plausible content. 
Our core idea is to exploit motion edges as guidance for completing the missing regions in the flow field. 
This better retains the piecewise-smooth nature of flow fields and leads to improved results.
In addition, we introduced using non-local flow connections to enable content propagation across motion boundaries.
We achieved seamless results by performing fusion of candidate pixels in the gradient domain.
We validated the efficacy of our method on DAVIS dataset under two settings and show that our method achieves a sizable performance boost over the state-of-the-art algorithms.



==> figure/fig_ablation_num_missing_pixels.tex <==
\begin{figure}[tp]
\centering
\includegraphics[width=0.7\columnwidth]{fig/num_missing_pixels_thres5.png}
% \includegraphics[width=\linewidth]{fig/num_missing_pixels_thres4.png}
\caption{\textbf{Number of missing pixels after each iteration.}
}
\label{fig:num_missing_pixels}
\end{figure}

==> figure/fig_comparison.tex <==
\begin{figure*}[t]

\mfigure{0.2}{{fig/comparison/object_removal/2/input.png}}\hfill % swing 00021
\mfigure{0.24}{{fig/comparison/object_removal/2/DFVI_canvas.png}}\hfill
\mfigure{0.24}{{fig/comparison/object_removal/2/OPN_canvas.png}}\hfill
\mfigure{0.24}{{fig/comparison/object_removal/2/ours_canvas.png}}\hfill

\mfigure{0.2}{{fig/comparison/fixed_region/1/input.png}}\hfill % bear 00008
\mfigure{0.24}{{fig/comparison/fixed_region/1/DFVI_canvas.png}}\hfill
\mfigure{0.24}{{fig/comparison/fixed_region/1/OPN_canvas.png}}\hfill
\mfigure{0.24}{{fig/comparison/fixed_region/1/ours_canvas.png}}\hfill

\mpage{0.23}{Input} \hfill
\mpage{0.23}{Xu~\etal~\cite{Xu-CVPR-DFVI}} \hfill
\mpage{0.23}{Oh~\etal~\cite{Oh-ICCV-Onion}} \hfill
\mpage{0.23}{Ours} \hfill


\caption{\textbf{Comparison of methods.}
}
\label{fig:comparison}
\end{figure*}



==> figure/fig_flow_comp_diffusion.tex <==
\begin{figure}[t]
\centering%
%
%
%
\newlength\ffca
%\setlength\ffca{5.7cm} % page-width size
\setlength\ffca{5.7cm} % column-width size
\newlength\ffcb
\setlength\ffcb{-0.8mm}
%
\parbox[t]{\ffca}{\centering%
  \fbox{\includegraphics[width=\ffca]{fig/flow_completion/flow_corrupted.png}}\\%
	\footnotesize (a) Input flow}%
%
\hfill%
%
\parbox[t]{\ffca}{\centering%
  \fbox{\includegraphics[width=\ffca]{fig/flow_completion/flow_completed_diffusion.png}}\\%
	\footnotesize (b) Completed flow with diffusion}%
%
\hfill%
%
\parbox[t]{\ffca}{\centering%
  \fbox{\includegraphics[width=\ffca]{fig/flow_completion/flow_completed.png}}\\%
	\footnotesize (c) Completed flow}%

\caption{
\textbf{Flow completion.}
(a) Optical flow estimated on the input video. Missing regions tend to have zero value (white).
(b) Completed flow, using diffusion).
(c) Piecewise-smooth completed flow, using the edges as guidance.}
\label{fig:flow_completion_diffusion}
\end{figure}



==> figure/fig_motivation.tex <==
\begin{figure*}[t]
\jbox{\textwidth}{0.3\linewidth}
\caption{Motivation of the method. Main idea.}
\label{fig:motivation}
\end{figure*}

==> table/ablation_flow.tex <==
\begin{table}[t]
    \scriptsize
    \caption{
    %
    \textbf{Ablation study on the flow completion methods.}
    %
    We report the average EPE, PSNR, SSIM and LPIPS results on DAVIS. 
    }
    \label{tab:ablation_flow}
    \centering
    % \resizebox{1\linewidth}{!} 
    % {
    \begin{tabular}{l cccc c cccc}
    %
    \toprule
    %
    & \multicolumn{4}{c}{Stationary masks} && \multicolumn{4}{c}{Object masks} \\
    %
    \cline{2-5} \cline{7-10}
    % 
    & Flow EPE $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ && Flow EPE $\downarrow$  & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
    %
    \midrule
    Diffusion                    & 1.79 & 30.18 & 0.9526 & 0.049 && 0.04 & 41.12 & 0.9902 & 0.008 \\
    Xu~\etal~\cite{Xu-CVPR-DFVI} & 2.01 & 27.17 & 0.9216 & 0.085 && 0.26 & 38.88 & 0.9882 & 0.009 \\
    Ours                         & 1.63 & 30.91 & 0.9564 & 0.048 && 0.03 & 41.89 & 0.9910 & 0.007 \\
    \bottomrule
    %
    \end{tabular}
    % }
\end{table}

==> table/ablation_gradient.tex <==
\begin{table}[t]
    % \scriptsize
    \caption{
    %
    \textbf{Ablation study on the propagation domain.}
    %
    We report the average PSNR, SSIM and LPIPS results on DAVIS. 
    }
    \label{tab:ablation_gradient}
    \centering
    % \resizebox{0.8\linewidth}{!} 
    % {
    \begin{tabular}{l ccc c ccc}
    %
    \toprule
    %
    & \multicolumn{3}{c}{Stationary screen-space masks} && \multicolumn{3}{c}{Synthetic object removal} \\
    %
    \cline{2-4} \cline{6-8}
    % 
    & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ && PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
    %
    \midrule
    % 
    color domain    & 28.47 & 0.9469 & 0.069 && 39.67 & 0.9897 & 0.009 \\
    % 
    gradient domain & 30.91 & 0.9564 & 0.048 && 41.89 & 0.9910 & 0.007 \\
    \bottomrule
    %
    \end{tabular}
    % }
\end{table}

==> table/ablation_nonlocal.tex <==
\begin{table}[t]
    \scriptsize
    \caption{
    %
    \textbf{Ablation study on the non-local temporal neighbors.}
    %
    We report the average PSNR, SSIM and LPIPS results on DAVIS.
    }
    \label{tab:ablation_nonlocal}
    \centering
    % \resizebox{1\linewidth}{!} 
    {
    \begin{tabular}{r ccc c ccc}
    %
    \toprule
    %
    & \multicolumn{3}{c}{Stationary screen-space masks} && \multicolumn{3}{c}{Synthetic object removal} \\
    %
    \cline{2-4} \cline{6-8}
    % 
    & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ && PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
    %
    \midrule
    % 
    w/o non-local neighbors & 30.78 & 0.9552 & 0.049 && 41.55 & 0.9907 & 0.007 \\
    % 
    w/ non-local neighbors  & 30.91 & 0.9564 & 0.048 && 41.89 & 0.9910 & 0.007 \\
    \bottomrule
    %
    \end{tabular}
    }
\end{table}
